Safe Planning for Articulated Robots Using Reachability-based Obstacle Avoidance With Spheres

Generating safe motion plans in real-time is necessary for the wide-scale deployment of robots in unstructured and human-centric environments. These motion plans must be safe to ensure humans are not harmed and nearby objects are not damaged. However, they must also be generated in real-time to ensure the robot can quickly adapt to changes in the environment. Many trajectory optimization methods introduce heuristics that trade-off safety and real-time performance, which can lead to potentially unsafe plans. This paper addresses this challenge by proposing Safe Planning for Articulated Robots Using Reachability-based Obstacle Avoidance With Spheres (SPARROWS). SPARROWS is a receding-horizon trajectory planner that utilizes the combination of a novel reachable set representation and an exact signed distance function to generate provably-safe motion plans. At runtime, SPARROWS uses parameterized trajectories to compute reachable sets composed entirely of spheres that overapproximate the swept volume of the robot's motion. SPARROWS then performs trajectory optimization to select a safe trajectory that is guaranteed to be collision-free. We demonstrate that SPARROWS' novel reachable set is significantly less conservative than previous approaches. We also demonstrate that SPARROWS outperforms a variety of state-of-the-art methods in solving challenging motion planning tasks in cluttered environments. Code, data, and video demonstrations can be found at \url{https://roahmlab.github.io/sparrows/}.

==> algorithms/pzsfo.tex <==
%~~~~~~~~~~~~ Compose SFO
\begin{algorithm}[t]
\small
\begin{algorithmic}[1]

\State $\pz{p_0}(\pzqi) \leftarrow \zeros$ %// initialize frame location 

\State$ \pz{R_0}(\pzqi) \leftarrow I_{3 \times 3}$ %// initialize frame orientation


\State\hspace{0in}{\bf for} $j = 1:\nq$ %// for each joint

    \State\hspace{0.2in}$\pz{R_{j}^{j-1}}(\pzqji), \pz{\nom{p\jssmu}} \leftarrow \pz{\homtrans_{j}^{j-1}}(\pzqji)$ as in \eqref{eq:homogeneous_transform}
    
    \State\hspace{0.2in}$\pz{p_j}(\pzqi) \leftarrow \pz{p_{j-1}}(\pzqi) \oplus \pz{R_{j-1}}(\pzqi) \pz{p_{j}^{j-1}}$
        
    \State\hspace{0.2in}$ \pz{R_j}(\pzqi) \leftarrow  \pz{R_{j-1}}(\pzqi)  \pz{R_{j}^{j-1}}(\pzqji)$ 
    
    \State\hspace{0.2in}$\pz{\FK_j}(\pzqi) \leftarrow \{ \pz{R_j}(\pzqi) ,  \pz{p_j}(\pzqi) \}$ 
    
\State\hspace{0in}{\bf end for}

\end{algorithmic}
\caption{\small $\{\pz{\FK_j}(\pzqi)\,:\, j \in \Nq \} = \texttt{PZFK}(\pzqi)$}
\label{alg:compose_sfo}
\end{algorithm}

==> algorithms/rdf_alg.tex <==
\begin{algorithm}[t]
\begin{algorithmic}[1]
\State $\{\pzqi\,:\, i \in \Nt\} \leftarrow (q_0,\dot q_0)$ 
\State $\co, \Go \leftarrow O$ 
\State{\bf for} $i = 1:n_t$ %// for each time steps
    \State\hspace{0.2in}{\bf for} $j = 1:n_q$ % for each joint
        \State\hspace{0.4in} $\pzFOjKi \leftarrow \texttt{PZFO}(\pzqi)$ 
        \State\hspace{0.4in} $\pzFOjki \leftarrow \texttt{slice}(\pzFOjKi, k)$ \label{lst:line:fo}
        \State\hspace{0.4in} $\pzFOjkibuf \leftarrow \pzFOjki\oplus Z_O^g$ \label{lst:line:buffered_fo}
    \State\hspace{0.2in}{\bf end for}
\State{\bf end for}
\State{\bf for} $j = 1:n_q$
    \State\hspace{0.2in} $\Pj \leftarrow \conv(\bigcup_{i = 1}^{\nt}\pzFOjkibuf)$ \label{lst:line:conv}
    %\State\hspace{0.2in} $\{(A_j^{(h)},b_j^{(h)})\,:\, h \in \Nhj\} \leftarrow \texttt{polytope}(\mathcal{P}_j)$
    \State\hspace{0.2in} {\bf if} $c_O \in \Pj$ {\bf then}
    % \State\hspace{0.2in} {\bf if} $A_j\,c_O-b_j \leq 0$ {\bf then} // $c_0 \in \mathcal{P}_j$
        %\State\hspace{0.4in} $\Tilde{r}_j \leftarrow \max_{h\in\Nhj}\frac{A_j^{(h)}\,p-b_j^{(h)}}{||A_j^{(h)}||}$ // negative distance 
        \State\hspace{0.4in} $\ardf_j \leftarrow -\dist(\co,\partial\Pj)$ // negative distance 
    \State\hspace{0.2in} {\bf else}
        %\State\hspace{0.4in} $\Tilde{r}_j \leftarrow \texttt{QP}\left(c_O, \{(A_j^{(h)},b_j^{(h)})\,:\, h \in \Nhj\}\right)$ // positive distance
        \State\hspace{0.4in} $\ardf_j \leftarrow \dist(\co,\partial\Pj)$ // positive distance 
    \State\hspace{0.2in} {\bf end if} 
\State{\bf end for}
\State \textbf{Return} $\{\ardf_j\,:\, j \in \Nq\}$
\end{algorithmic}
\caption{\texttt{RDF}$(q_0, \dot q_0, k, O)$}
\label{alg:rdf}
\end{algorithm}

==> algorithms/vertex_enumeration.tex <==
\begin{algorithm}[t]
    \caption{Zonotope Vertex Enumeration}
    \label{alg:vertex_enumeration}
    \begin{algorithmic}[1]
        \REQUIRE Zonotope $Z \subset \mathbb{R}^2$ with $n \in \mathbb{N}$ generators $g_1, \cdots, g_n$ \jon{should 1 and 2 be under required?}
        \STATE \quad Multiply any generator with negative y-value by $-1$.
        \STATE \quad Reduce generators $g_1, \cdots, g_n$ to $g\prime_1, \cdots, g\prime_m$ by\\
        \quad  summing generators with the same direction $(m \leq n)$.
        \STATE \quad Sort $g\prime_1, \cdots, g\prime_m$ by angle in ascending order. 
        \STATE \quad Compute vertex coefficient matrix $C \in \mathbb{R}^{m \times m}$ such that
        \begin{equation*}
            C(i,j) = 
            \begin{cases}
                1 & \text{if } j \geq i \\
                -1 & \text{otherwise}
            \end{cases}.
        \end{equation*}
        \STATE \quad  Compute the $2m$ vertices $\{v_1, \cdots, v_{2m}\}$:
        \begin{align*}
            v_k &= c + \sum_{j=1}^{m} C(k,j) g_j \\
            v_{m+k} &= c - \sum_{j=1}^{m} C(k,j) g_j. 
       \end{align*}
        \STATE \textbf{End}
    \end{algorithmic}
\end{algorithm}

==> sections/approach.tex <==
\section{Reachability-based Signed Distance Function}\label{sec:approach}

\subsection{Signed Distance Between Zonotopes}
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\columnwidth]{figures/buffer_obstacle.pdf}
    \caption{Illustration of signed distance for convex polytopes. In particular, this works well with zonotopes.\jon{Add labels. Highlight pos/neg distance better.}} 
    \label{fig:zono_sdf}
    \vspace*{-0.2cm}
\end{figure}
In this section we describe how to compute signed distance between two zonotopes, how to represent this function exactly using a ReLU neural network, and how we leverage this novel representation for representing obstacle-avoidance constraints for safe motion planning.

\begin{defn}\label{defn:zono_pentration_depth}
    The \defemph{penetration depth} of $Z_1$ and $Z_2$ in $\R^{\nd}$ is denoted $\pi(Z_1, Z_2)$ and is defined by 
    \begin{equation}
        \pdf(Z_1, Z_2) = \min \{\|t\| :\ \text{int}(Z_1 + t \cap Z_2) = \emptyset, \quad t \in \R^{\nd}\}.
    \end{equation}
\end{defn}


\begin{lem}\label{lem:zono_sdf}
Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. 
Then the signed distance between $Z_1$ and $Z_2$ is given by
\begin{equation}
    \sdf(Z_1, Z_2)  = 
        \begin{cases}
          \dist(c_1; Z_{2,buf})  & \text{if } c_1 \not \in Z_{2,buf} \\
          -\pdf(c_1, Z_{2,\text{buf}}) & \text{if } c_1 \in Z_{2,buf}
        \end{cases} .
\end{equation}
\end{lem}
\begin{proof} See \cite{michaux2023rdf}.
\end{proof}

Maybe say something about how this can be solved using a convex optimization program.
But here, we instead compute the distances exactly.


\begin{lem} \label{lem:hyperplane_distance}
We can compute the distance  
\end{lem}
\begin{proof} Let 
\begin{equation}
    h_i(t) = v_1 + s (v_2 - v_1) 
\end{equation}
for $s \in [0,1]$.

The distance between a point and the line segment is
\begin{equation}
    \phi_i(s) = \|h_i(s) - p\|^2
\end{equation}

\begin{equation}
    \hat{s}_i = \frac{(p - v_1)^T(v_2 - v_1)}{(v_2 - v_1)^T (v_2 - v_1)}
\end{equation}

\begin{equation}
    s^{\ast}_i = \min (\max (\hat{s}_i, 0), 1)
\end{equation}
\end{proof}

\begin{thm} \label{thm:exact_sdf}
The distance between two zonotopes can be computed
\end{thm}
\begin{proof}
\end{proof}
Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.
We use this to build the neural network in the next section
\subsection{Neural Network Architecture}

\begin{thm}
\label{thm:network_bound}
\end{thm}
\begin{proof}
\end{proof}


% Before proving the required result, we prove several intermediate results. 
% \subsection{Signed Distance Between Zonotopes}
% \label{subsec:sdf_zono}

% Here we derive the signed distance between two zonotopes.
% To proceed we first require a condition for determining if two zonotopes are in collision:
% \begin{lem}\label{lem:zono_intersection}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes. Then $Z_1 \cap Z_2 \neq \emptyset$ if and only if $c_1 \in Z_{2,\text{buf}} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
% Suppose the intersection of $Z_1$ and $Z_2$ is non-empty. This is equivalent to the existence of $z_1 \in Z_1$ and $z_2 \in Z_2$ such that $z_1 = z_2$. Furthermore, by definition of a zonotope (Defn. \ref{defn:zonotope}), this is equivalent to the existence of coefficients $\beta_1$ and $\beta_2$ such that $z_1 = c_1 + G_1 \beta_1$, $z_2 = c_2 + G_2 \beta_2$, and
% \begin{align}
%     &c_1 + G_1 \beta_1 = c_2 + G_2 \beta_2 \\
%     \iff& c_1 = c_2 + G_2 \beta_2 - G_1 \beta_1 \\
%     \iff& c_1 \in (c_1, G_1 \cup G_2) = Z_{2, \text{buf}}.
% \end{align}
% Thus we have shown that $Z_1 \cap Z_2 \neq \emptyset$ if and only if $c_1 \in (c_1, G_1 \cup G_2) = Z_{2, \text{buf}}$.
% \end{proof}

% Lemma \ref{lem:zono_intersection} can then be used to compute the the positive distance between two non-intersecting zonotopes:
% \begin{lem}\label{lem:zono_positive_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be non-intersecting zonotopes.
% \begin{align}
%     \dist(Z_1, Z_2) = \dist(c_1; Z_{2,buf})
% \end{align}
% where $Z_{2,\text{buf}} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
% Suppose $Z_1$ and $Z_2$ are non-intersecting zonotopes such that $\dist(Z_1, Z_2) = r$ for some $r \in \mathbb{R}^{+}$. That is, there exists $z_1 \in Z_1$ and $z_2 \in Z_2$ such that 
% \begin{align}
%     r &= \|z_1 - z_2\| \\
%     &= \|c_1 + G_1 \beta_1 - (c_2 + G_2 \beta_2) \| \\
%     &= \| c_1 - (c_2 + G_2 \beta_2 = G_1 \beta_1) \| \\
%     &\geq \dist(c_1, (c_2, G_1 \cup G_2)) \\
%     &= \dist(c_1, Z_{2, \text{buf}}).
% \end{align}
% Now suppose $\dist(c_1, Z_{2, \text{buf}}) = r$. Then there exists coefficients $\beta_1$ and $beta_2$ such that
% \begin{align}
%     r &= \|c_1 - (c_2 + G_1 \beta_1 + G_2 \beta_2) \| \\
%     &= \|c_1 - G_1 \beta_1 - (c_2 + G_2 \beta_2) \| \\
%     &= \|z_1 - z_2\| \\
%     &\geq \dist(Z_1, Z_2).
% \end{align}
% Together, these inequalities prove that $\dist(Z_1, Z_2) = \dist(c_1; Z_{2,buf})$.
% \end{proof}
% Let $\text{int}(S)$ denote the interior of a set.
% Before deriving the negative distance we first define the penetration depth  \cite{cameron1986mtd} of two zonotopes:
% \begin{defn}\label{defn:zono_pentration_depth}
%     The \defemph{penetration depth} of $Z_1$ and $Z_2$ in $\R^{\nd}$ is denoted $\pi(Z_1, Z_2)$ and is defined by 
%     \begin{equation}
%         \pdf(Z_1, Z_2) = \min \{\|t\| :\ \text{int}(Z_1 + t \cap Z_2) = \emptyset, \quad t \in \R^{\nd}\}.
%     \end{equation}
% \end{defn}

% The penetration depth $\pi(Z_1,Z_2)$ can be interpreted as the minimum translation applied to $Z_1$ such that the interior of $Z_1 \cap Z_2$ is empty.
% Following \cite{agarwal2000convex} we can now redefine the penetration distance between $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ in terms of $c_1$ and $Z_{2,\text{buf}}$.
% \begin{lem}\label{lem:zono_negative_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$.
% Then the penetration depth between $Z_1$ and $Z_2$ is given by
%    \begin{align}
%      \pdf(Z_1, Z_2) = \pi(c_1, Z_{2,\text{buf}}),
% \end{align} 
% \end{lem}
% \begin{proof}
% Suppose $Z_1 \cap Z_2 \neq \emptyset$. 
% Then by Defn. \ref{defn:zono_pentration_depth}, there exists a translation vector $t \in \R^{\nd}$ such that $\text{int}(Z_1 + t \cap Z_2) = \emptyset$. 
% This means that $Z_1$ is translated by $t$ such that only the boundaries of $Z_1 + t$ and $Z_2$ are intersecting. 
% Thus, there exists $z_1 \in \partial Z_1$ and $z_2 \in \partial Z_2$ such that $z_1 + t = z_2$. 
% Furthermore, there exist coefficients $\beta_1$ and $\beta_2$ such that $z_1 = c_1 + G_1 \beta_1$, $z_2 = c_2 + G_2 \beta_2$, and
% \begin{align}
%     & c_1 + G_1 \beta_1 + t = c_2 + G_2 \beta_2 \\
%     \iff& c_1 + t = c_2 + G_2 \beta_2 - G_1 \beta_1 \in \partial Z_{2,\text{buf}}.
% \end{align}
% Since $\pi(c_1, Z_{2,\text{buf}})$ is the minimum distance between $c_1$ and all points in $\partial Z_{2,\text{buf}}$, this means that $\pi(c_1, Z_{2,\text{buf}}) \leq \|t\|$.

% Now suppose $c_1 \in Z_{2, \text{buf}}$.
% Let $t \in \R^{\nd}$ such that $\|t\|$ is the penetration depth of $c_1$ and $Z_{2,\text{buf}}$. 
% Then there exists coefficients $\beta_1$ and $\beta_2$ such that $z_2 = c_2 + G_1 \beta_1 + G_2 \beta_2$ and
% \begin{align}
%     c_1 + t = c_2 + G_1 \beta_1 + G_2 \beta_2 \\
%     c_1 -G_1 \beta_1 + t = c_2 + G_2 \beta_2.
% \end{align}
% This means translating $z_1 = c_1 - G_1 \beta_1 \in \partial Z_1$ by $t$ causes the boundary of $Z_1$ to intersect the boundary of $Z_2$. 
% Therefore $\pi(Z_1, Z_2) \leq \|t\|$.
% Together the above inequalities prove the result.
% \end{proof}

% \begin{thm}\label{thm:zono_sdf}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. 
% % Denote $\mathcal{P} = \bigcap_{i}\mathcal{H}_i$ as the half-space representation of the buffered zonotope $Z_{2,buf} = (c_2, G_1 \cup G_2)$.
% Then the signed distance between $Z_1$ and $Z_2$ is given by
% \begin{equation}
%     \sdf(Z_1, Z_2)  = 
%         \begin{cases}
%           \dist(c_1; Z_{2,buf})  & \text{if } c_1 \not \in Z_{2,buf} \\
%           -\pdf(c_1, Z_{2,\text{buf}}) & \text{if } c_1 \in Z_{2,buf}
%         \end{cases} .
% \end{equation}
% \end{thm}
% \begin{proof} The proof follows readily from Lemmas \ref{lem:zono_positive_distance} and \ref{lem:zono_negative_distance}.
% \end{proof}

% Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.

% \subsection{The Proof}

% We prove the desired result by considering two cases. 
% First assume  $O \cap \FO(q(T;k)) = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(O, \FO(q(T;k))) &= \underset{t \in T}{\min}\: \underset{j \in \Nq}{\min}\:  \sdf(O, \FO_j(q(t;k))) \\
%     &\geq \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\:  \sdf(O, \pzFOjki) \\
%     % &= \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\: \sdf(O, \pzFOjkibuf) \\
%     &= \underset{i \in \Nt}{\min}\: \underset{j \in \Nq}{\min}\: \sdf(\co, \pzFOjkibuf) \\
%     &= \underset{j \in \Nq}{\min}\: \sdf(\co, \bigcup_{i\in\Nt} \pzFOjkibuf) \\
%     &\geq \underset{j \in \Nq}{\min}\: \sdf(\co, \Pj) \\
%     &= \underset{j \in \Nq}{\min}\: \ardf_j(\co, \Pj) \\
%     &= \ardf(\co, \bigcup_{j\in \Nq} \Pj),
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Lemma \ref{lem:pz_FO}, the third equality follows from Lemma \ref{lem:zono_positive_distance}, the fourth inequality by flipping the order of minimization, and the fifth inequality follows from Def. \ref{def:convhull}. 

% Thus $\ardf$ underapproximates the distance between the forward occupancy and the obstacle. 
% If instead $O \cap \FO_j(\q) \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that we can overapproximate the penetration distance between an obstacle and the forward occupancy.

% \begin{lem}\label{lem:zono_negative_distance}
% Let $Z_1 = (c_1, G_1)$ and $Z_2 = (c_2, G_2)$ be zonotopes such that $Z_1 \cap Z_2 \neq \emptyset$. Denote $\mathcal{P} = \bigcap_{i}\mathcal{H}_i$ as the half-space representation of the buffered zonotope $Z_{2,buf} = (c_2, G_1 \cup G_2)$. Then the penetration depth of $Z_1$ and $Z_2$ is
%    \begin{align}
%      \pi(Z_1, Z_2) = \underset{i}{\min}\:\dist(c_1, \mathcal{H}_i),
% \end{align} 
% where $\mathcal{P}$ is the polytope representation of $Z_{2,buf} = (c_2, G_1 \cup G_2)$.
% \end{lem}
% \begin{proof}
%     See Appendix.
%     % It is readily apparent that
%     % \begin{align}
%     %     \pi(Z_1, Z_2) = \pi(c_1, Z_{2,buf}).
%     % \end{align}
% \end{proof}


\subsection{Algorithm}
\input{algorithms/redefine_alg}
\begin{itemize}
    \item Will probably want to 
\end{itemize}


==> sections/old/06_network.tex <==
\section{Exact SDF with ReLU Networks}




















%~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~~ OLD STFF


\label{sec:nnsdf}
The Section \ref{sec:sfo} described how to construct the .
Because this representation is composed of spheres, it is straightforward to use with a signed distance function.
This section first describes how to compute the signed distance function exactly between a zonotope and a point in 3D. between two zonotopes, how to represent this function exactly using a ReLU neural network, and how we can replace the obstacle-avoidance constraints in \opt with a novel neural implicit representation that overapproximates the distance between the forward occupancy of the ego vehicle and obstacles in the environment.



\subsection{Exact Signed Distance Between a Point and a Zonotope}
\label{subsec:rdf_derivation}
% We start by stating a result about the signed distance between two zonotopes: \jinsun{Pls use calligraphic font for sets...}
% \jon{Why?}

% \begin{lem}\label{lem:zono_sdf}
% Let $Z = (\cz, \Gz)$ and $O = (\co, \Go)$ be zonotopes and define $\Oz = (\cz, \Gz \cup \Go)$ \jinsun{$\Gz \cup \Go$ seems a wrong math expression to me. and the lower case $z$ is the vehicle state...} as the zonotope $O$ buffered by the generators of $Z$.
% Then the signed distance \jinsun{you are assuming the reader knows what it is} between $Z$ and $O$ is given by \jinsun{define $\partial$}
% \begin{equation}
%     \sdf(Z, O)  = 
%         \begin{cases}
%           \dist(\cz; \partial \Oz)  & \text{if } Z \cap O =  \emptyset \\
%           -\dist(\cz; \partial  \Oz) & \text{if } Z \cap O \neq \emptyset 
%         \end{cases}, \label{eq:sdf}
% \end{equation}
% where
%     \begin{equation}
%        \dist(\cz; \partial \Oz) = \min_{x \in \partial \Oz} \|\cz - x\|. \label{eq:boundary_distance}
%     \end{equation}
% \end{lem}
% \begin{proof}
% See \cite[Theorem 19]{michaux2023rdf}. 
% \end{proof}

The following theorem leverages the properties of zonotopes to find a closed form expression for the exact signed distance between a collection of zonotopes:
\begin{thm} \label{thm:exact_zono}
Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes in $\R^2$ for each $j \in \J$ where $\J$ has a finite number of elements in it.
Let $\Obs = \bigcup_{j \in \J} \Oj$.
Let $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
Suppose that for each $j \in \J$, $\Ojz$ has $N_j$ vertices.
Let $V_j$ be the set of vertices of $\Ojz$ ordered in counterclockwise fashion and $\{h_{i,j}\}_{i=1}^{N_j}$ be the set of line segments between consecutive vertices in $V_j$.

The signed distance between $\Z$ and $\Obs$ is given by 
\begin{align}
   \hspace*{-0.48cm} \sdf(\Z, \Obs)
    % &= \underset{j \in \J}{\min}\: \sdf(Z; \Oj) \nonumber \\
    &=
    \begin{cases}
          \underset{j \in \J}{\min}\: \underset{i \in \{1,\ldots,N_j\} }{\min}\: \dist(\cz; h_{i,j})  & \text{if } \Z \cap \Obs =  \emptyset \\
          -\underset{j \in \J}{\min}\: \underset{i\in \{1,\ldots,N_j\}}{\min}\: \dist(\cz; h_{i,j}) & \text{if } \Z \cap \Obs  \neq \emptyset 
    \end{cases}.  \label{eq:rdf}
\end{align}
% \begin{equation}\label{eq:zonotope_sdf_eq}
%     \sdf(\Z, \mathcal{O}) = 
%         \begin{cases}
%           \underset{i\in \{1,\ldots,N\}}{\min}\: \dist(\cz; h_i)  & \text{if } \Z \cap \mathcal{O} =  \emptyset \\
%           \underset{i\in \{1,\ldots,N\}}{-\min}\: \dist(\cz; h_i) & \text{if } \Z \cap \mathcal{O} \neq \emptyset 
%         \end{cases} .
% \end{equation}
\end{thm}
\begin{proof} 
Assume without loss of generality that $\Z \cap \Oj =  \emptyset$. 
Note that $\sdf(\Z,\Oj) = \dist(\cz; \partial \Ojz)$ because of \cite[Theorem 19]{michaux2023rdf}.
Because $\partial \Ojz = \{ h_{i,j} \}_{i=1}^{N_j}$, the result follows by taking the minimum over $j \in \J$.
The proof for the case $Z \cap \Obs \neq \emptyset$ is similar.
Fig. \ref{fig:zono_sdf} illustrates this proof when the distance is being computed between two zonotopes. 
\end{proof}
Because of Assumptions \ref{ass: offline reachability} and \ref{ass: obs in T}, one can apply Theorem \ref{thm:exact_zono} to compute the constraint in $\opt$. 
However, because \eqref{eq:rdf} still requires computing the distance between a vertex and a finite length line segment, it naively would still require solving a convex quadratic program. 


% In the following theorem, we leverage properties of zonotopes to find a closed form expression for the exact signed distance between two zonotopes:
% \begin{thm} \label{thm:exact_sdf}
% Let $\Z = \zonocg{\cz}{\Gz}$ and $\mathcal{O} = \zonocg{\co}{\Go}$ be zonotopes in $\R^2$ and define $\mathcal{O}_z = \zonocg{c_o}{[\Gz,\Go]}$.
% Suppose $\Oz$ has $N$ vertices, and let $V$ be the set of vertices of $\Oz$ ordered in counterclockwise fashion and $\{h_i\}_{i=1}^N$ be the set of corresponding line segments between consecutive vertices in $V$. 
% Then the signed distance between $\Z$ and $\mathcal{O}$ is
% \begin{equation}\label{eq:zonotope_sdf_eq}
%     \sdf(\Z, \mathcal{O}) = 
%         \begin{cases}
%           \underset{i\in \{1,\ldots,N\}}{\min}\: \dist(\cz; h_i)  & \text{if } \Z \cap \mathcal{O} =  \emptyset \\
%           \underset{i\in \{1,\ldots,N\}}{-\min}\: \dist(\cz; h_i) & \text{if } \Z \cap \mathcal{O} \neq \emptyset 
%         \end{cases} .
% \end{equation}
% \end{thm}
% \begin{proof} 
% Assume without loss of generality that $\Z \cap \mathcal{O} =  \emptyset$. 
% Note that $\sdf(\Z, \mathcal{O}) = \dist(\cz; \partial \Oz)$ because of \cite[Theorem 19]{michaux2023rdf}.
% Because $\partial \Oz = \{ h_i \}_{i=1}^N$, the result follows. 
% % Let $h_i$ be a given line segment comprising the boundary of $\Oz$ and let $\vi{1}$ and $\vi{2}$ be its corresponding ordered vertices. 
% % Then we can parameterize the line containing $h_i$ in terms of $\tau \in \mathbb{R}$ as
% % \begin{equation}
% %     H_i(\tau) = \vi{1} + \tau (\vi{2} - \vi{1})
% % \end{equation}
% % such that $H_i(\tau)$ is on the line segment $h_i$ if $\tau \in [0,1]$. 
% % Then the distance between $c_1$ and $h_i$ can be found by considering  
% % \begin{equation}
% %     \phi_i(\tau) = \|H_i(\tau) - \cz\|_{2} .
% % \end{equation}
% % We can find the minimum of $\phi_i^{2}(\tau)$ and solve for the value $\hat{\tau}_i$ where its gradient vanishes:
% % \begin{equation}
% %     \hat{\tau}_i = \frac{(\cz - \vi{1})^T(\vi{2} - \vi{1})}{(\vi{2} - \vi{1})^T (\vi{2} - \vi{1})}. \label{eq:line_projection}
% % \end{equation}
% % The value $\hat{\tau}_i$ may not be on the line segment $h_i$, so we project it onto the interval $[0,1]$ to get
% % \begin{equation}
% %     \tau^{\ast}_i = \min (\max (\hat{\tau}_i, 0), 1). \label{eq:segment_projection}
% % \end{equation}
% % Then it is clear that $\phi_i(t^{\ast}_i) = \dist(\cz; h_i)$ \jinsun{$\phi_i(\tau^{\ast}_i)$?}.
% % Therefore the distance between $Z$ and $O$ is the minimum distance between $\cz$ and all line segments $h_i$ comprising the boundary of $\Oz$: 
% % \begin{align}
% %     \dist(Z; O) 
% %     &= \dist(\cz; \Oz) \nonumber  \\
% %     &= \underset{i}{\min}\: \phi_i(\tau^{\ast}_i) \nonumber \\ 
% %     &= \underset{i}{\min}\: \dist(\cz; h_i) .  \label{eq:dist}
% % \end{align}
% % % \begin{equation}
% % %     \dist(Z; O) 
% % %     = \dist(\cz; \Oz)
% % %     = \underset{i}{\min}\: \phi_i(\tau^{\ast}_i) 
% % %     = \underset{i}{\min}\: \dist(\cz; h_i) .  \label{eq:dist}
% % % \end{equation}
% The proof for the case $Z \cap \Obs \neq \emptyset$ is similar.
% \end{proof}

% Note that we provide a visual illustration of this theorem in Fig. \ref{fig:zono_sdf}.
% We next show that this result extends to computing the signed distance to a collection of zonotopes.
% \begin{cor}
% Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes and define $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
% Denote $\Obs = \underset{j}{\bigcup} \Ojz$.
% Then the signed distance between $Z$ and $\Obs$ is given by 
% \begin{align}
%     \sdf(Z; \Obs) &= \underset{j}{\min}\: \sdf(Z; \Oj) \nonumber \\
%     &=
%     \begin{cases}
%           \underset{j}{\min}\: \underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } Z \cap \Obs =  \emptyset \\
%           -\underset{j}{\min}\: \underset{i}{\min}\: \dist(\cz; h_{i,j}) & \text{if } Z \cap \Obs  \neq \emptyset 
%     \end{cases} ,  \label{eq:rdf}
% \end{align}
% where $\cz$ is the center of $Z$ and $h_{i,j}$ is the $i^{th}$ line segment for $\Ojz$.
% \end{cor}
% \begin{proof}
%     The result follows trivially from Theorem \ref{thm:exact_sdf}.
% \end{proof}

% \begin{figure}[t]
%     \centering
%     \includegraphics[width=0.8\columnwidth]{figures/redefine_buffer_obstacle.pdf}
%     \caption{Graphical illustration of signed distance between zonotopes. (Top) The top row illustrates the positive distance function between two zonotopes. First, the gray zonotope is buffered by the generators of the purple zonotope. Then, the distance is computed between the purple zonotope's center and the closest line segment of the buffered zonotope. (Bottom) The bottom row graphically illustrates the negative distance between two zonotopes. First, the pink zonotope's generators buffer the gray zonotope. Then, the negative distance is computed by projecting the pink zonotope's centers on each of the buffered zonotope's half-spaces.} 
%     \label{fig:zono_sdf}
%     \vspace*{-0.2cm}
% \end{figure}

% By using the previous theorem, the next result describes how to compute the distance between the ego vehicle and obstacles.\jon{reword?}
% \begin{thm} \label{thm:exact_rdf}
%     Suppose the ego vehicle is starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$.
%     Let $\xi$ and $\vartheta$ be the zonotope reachable set and zonotope obstacle representation as in Assumptions \ref{ass: offline reachability} and \ref{ass: obs in T}, respectively. 
%     Then $\rdf(\xi(z_0,p), \vartheta(k)) \leq \rdf( \{\E\big(t,z_0,p\big)\}_{t\in T}, \{\Obskt\}_{t \in T})$. 
% \end{thm}
% \begin{proof}We prove the desired result by considering two cases. 
% First assume  $\FOt \cap \Obst  = \emptyset$ for all $t \in T$ and let $\FOT = \{\E\big(t,z_0,p\big)\}_{t\in T}$ and $\ObskT = \{\Obskt\}_{t \in T}$.
% Then
% \begin{align}
%     \rdf(\FOT, \ObskT) &= \min_{t \in T} \sdf(\FO\big(t,z_0,p\big), \Obskt) \\
%     &\geq \underset{j \in \J}{\min}\: \sdf(\FOzj \big(z_0,p\big), \vartheta(j,k)) \\
%     &= \underset{j \in \J}{\min}\: \underset{i\in \{1,\ldots,N_j\}}{\min}\: \dist(\cj; h_{i,j}) \\
%     &= \underset{j \in \J}{\min}\: \rdf(\xi(z_0,p), \vartheta(j,k)) \\
%     &= \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj)
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Assumption \ref{ass: offline reachability}, the third equality follows from Theorem \ref{thm:exact_sdf}, the fourth \stkout{inequality} \new{equality} by flipping the order of minimization. 
% Thus $\ardf$ underapproximates the positive distance between the forward occupancy and an obstacle. 

% If instead $\FOt \cap \Obst \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that $\ardf$ overrapproximates the negative distance between an obstacle and the forward occupancy.
% \jon{should the negative distance be an underapproximation too?} \jinsun{I think it is an overapproximation in the negative case}
% \end{proof}
% \begin{thm} \label{thm:exact_rdf}
%     Suppose the ego vehicle is starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$.
%     Consider an obstacle $\Obst$ with a zonotope representation.
%     Let $\{\FOzj\}$ \jinsun{mention Assumption 7 here?} be the zonotope reachable set overapproximating the ego vehicle's trajectory.
%     Define $\ardf_j$ as the following: \jon{reword}
%     \begin{equation}
%     \label{eq:ardf_j}
%     \ardf_j(\FOzj; \Obszj) = 
%         \begin{cases}
%           \underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  =  \emptyset \\
%           -\underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  \neq  \emptyset,
%         \end{cases} 
%     \end{equation}
%     \jinsun{$\Obszj$? conflict with Defintion 5}
%     where $\cj$ \jinsun{where is it used?} is the center of zonotope $\FOzj$, and $h_{i,j}$ is the $i^{th}$ line segment of the obstacle zonotope buffered by the generators of $\FOzj$.
%     Now define the function $\ardf$ as:
%     \begin{equation}
%     \label{eq:ardf}
%         \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) = \underset{j \in \J}{\min}\ardf_j(\FOzj; \Obszj).
%     \end{equation}
% If $\FOT \cap \ObsT = \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \leq \rdf(\FOT; \ObsT)$.
% If $\FOT \cap \ObsT \neq \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \geq \rdf(\FOT; \ObsT)$.
% \end{thm}
% \begin{proof}We prove the desired result by considering two cases. 
% First assume  $\FOt \cap \Obst  = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(\FOT; \ObsT) &= \min_{t \in [0, \tf]} \sdf(\FO\big(t,z_0,p\big); \Obst) \\
%     &\geq \underset{j \in \J}{\min}\: \sdf(\FOzj \big(z_0,p\big); \Obszj) \\
%     &= \underset{j \in \J}{\min}\: \underset{i \in \I}{\min}\: \dist(\cj; h_{i,j}) \\
%     &= \underset{j \in \J}{\min}\: \ardf_j(\FOzj; \Obszj) \\
%     &= \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj)
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Assumption \ref{ass: offline reachability}, the third equality follows from Theorem \ref{thm:exact_sdf}, the fourth \stkout{inequality} \new{equality} by flipping the order of minimization. 
% Thus $\ardf$ underapproximates the positive distance between the forward occupancy and an obstacle. 

% If instead $\FOt \cap \Obst \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that $\ardf$ overrapproximates the negative distance between an obstacle and the forward occupancy.
% \jon{should the negative distance be an underapproximation too?} \jinsun{I think it is an overapproximation in the negative case}
% \end{proof}


% For this result to be useful, we need to extend it to multiple zonotopes, which we do next:



% \subsection{Main Theorem}
% \jon{Is this the main theorem?}
% In this subsection we introduce the main theorem used to compute the exact distance between approximation to the reachability-based distance function.
% \stkout{In this section w}\new{W}e derive an approximation to the true RDF using zonotope arithmetic.
% We start by defining a distance function between  \jinsun{unfinished sentence}
% \begin{defn}\label{def:rdf_point}
% Given initial condition $z_0\in\Z_0$ and control parameter $p\in\PP$, the \defemph{reachability-based distance} function associated with the forward occupancy \stkout{$\FOt$} \new{$\E\big(t,z_0,p\big)$} \jinsun{it contradicts with the definition of $\E$ in \eqref{eq: def occupancy}} \challen{Fixed} of the ego vehicle and obstacle $\Obst$ \jinsun{So obstacles are no longer indexed?} over the interval $T = [0, \tf]$ is a mapping defined by
% \begin{equation}
%     \rdf(\FOT; \ObsT) = \min_{t \in [0, \tf]} \sdf(\FO\big(t,z_0,p\big); \Obst).
% \end{equation}
% \jinsun{$\FOT$ is improper because by definition $\E$ cannot take an interval as its argin}
% \jon{why not?}
% \end{defn}
% By using zonotopes, the next theorem approximates the distance between the ego vehicle and obstacles.\jon{reword}

% \begin{thm} \label{thm:exact_rdf}
%     Suppose the ego vehicle is starting from initial condition $z_0\in\Z_0$ with control parameter $p\in\PP$ and satisfies \eqref{eq: dyn tilde_z} for all $t \in [0, \tf]$.
%     Consider an obstacle $\Obst$ with a zonotope representation.
%     Let $\{\FOzj\}$ \jinsun{mention Assumption 7 here?} be the zonotope reachable set overapproximating the ego vehicle's trajectory.
%     Define $\ardf_j$ as the following: \jon{reword}
%     \begin{equation}
%     \label{eq:ardf_j}
%     \ardf_j(\FOzj; \Obszj) = 
%         \begin{cases}
%           \underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  =  \emptyset \\
%           -\underset{i}{\min}\: \dist(\cz; h_{i,j})  & \text{if } \FOzj \cap \Obszj  \neq  \emptyset,
%         \end{cases} 
%     \end{equation}
%     \jinsun{$\Obszj$? conflict with Defintion 5}
%     where $\cj$ \jinsun{where is it used?} is the center of zonotope $\FOzj$, and $h_{i,j}$ is the $i^{th}$ line segment of the obstacle zonotope buffered by the generators of $\FOzj$.
%     Now define the function $\ardf$ as:
%     \begin{equation}
%     \label{eq:ardf}
%         \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) = \underset{j \in \J}{\min}\ardf_j(\FOzj; \Obszj).
%     \end{equation}
% If $\FOT \cap \ObsT = \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \leq \rdf(\FOT; \ObsT)$.
% If $\FOT \cap \ObsT \neq \emptyset$, then $\ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj) \geq \rdf(\FOT; \ObsT)$.
% \end{thm}
% \begin{proof}We prove the desired result by considering two cases. 
% First assume  $\FOt \cap \Obst  = \emptyset$ for all $t \in T$. 
% Then
% \begin{align}
%     \rdf(\FOT; \ObsT) &= \min_{t \in [0, \tf]} \sdf(\FO\big(t,z_0,p\big); \Obst) \\
%     &\geq \underset{j \in \J}{\min}\: \sdf(\FOzj \big(z_0,p\big); \Obszj) \\
%     &= \underset{j \in \J}{\min}\: \underset{i \in \I}{\min}\: \dist(\cj; h_{i,j}) \\
%     &= \underset{j \in \J}{\min}\: \ardf_j(\FOzj; \Obszj) \\
%     &= \ardf(\underset{j \in \J}{\cup} \FOzj; \underset{j \in \J}{\cup} \Obszj)
% \end{align}
% where the first equality follows from the definition of $\rdf$ in Def. \ref{def:rdf_point}, the second inequality follows from Assumption \ref{ass: offline reachability}, the third equality follows from Theorem \ref{thm:exact_sdf}, the fourth \stkout{inequality} \new{equality} by flipping the order of minimization. 
% Thus $\ardf$ underapproximates the positive distance between the forward occupancy and an obstacle. 

% If instead $\FOt \cap \Obst \neq \emptyset$ for some $t \in T$, replacing $\geq$ with $\leq$ shows that $\ardf$ overrapproximates the negative distance between an obstacle and the forward occupancy.
% \jon{should the negative distance be an underapproximation too?} \jinsun{I think it is an overapproximation in the negative case}
% \end{proof}

\subsection{Neural Network Architecture}
\label{subsec:nn_architecture}
We now use results from Section \ref{subsec:rdf_derivation} to enable the closed form expression of the signed distance function between zonotopes.
In particular, we show that the signed distance between collections of zonotopes can be computed exactly with an implicit neural network with fixed, prespecified weights.
% We then generalize the network to compute the signed distance to a collection of zonotopes.
% between the forward occupancy of the ego vehicle and obstacles in the environment
Before constructing this network, we note the following observation about max and min operations which was proven in \cite[Lemma D.3]{arora2016} \cite[Section 3.2]{ferlez2020}:

\begin{lem}\label{lem:minmax}
% Let $W ^{\min}, b ^{\min},W ^{\max},$ and $b ^{\max}$ be defined as:
% % The functions $\min(x,y)$ and $\max(x,y)$ can be specified as ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$ such that
% \begin{align}
%     W ^{\min} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             1 & -1 \\
%             -1 & 1 \\
%             -1 & -1
%     \end{bmatrix},
%     b^{\min} = 
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & -\frac{1}{2} & -\frac{1}{2}
%     \end{bmatrix}
% \end{align}
% \begin{align}
%     W^{\max} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             -1 & -1 \\
%             -1 & 1 \\
%             1 & -1
%     \end{bmatrix},
%      b^{\max} =
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & \frac{1}{2} & \frac{1}{2}
%     \end{bmatrix}.
% \end{align}
The maximum or minimum of a pair of numbers can be computed using a ReLU network with width of $4$ and a depth of $2$ as:
\begin{align}
\min(x,y) &= \relu \left(   \begin{bmatrix}
            1 & 1 \\
            1 & -1 \\
            -1 & 1 \\
            -1 & -1
    \end{bmatrix} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T  \begin{bmatrix}
        \frac{1}{2} \\ -\frac{1}{2} \\ -\frac{1}{2} \\ -\frac{1}{2}
    \end{bmatrix} \\ 
\max(x,y) &= \relu \left(  \begin{bmatrix}
            1 & 1 \\
            -1 & -1 \\
            -1 & 1 \\
            1 & -1
    \end{bmatrix} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T\begin{bmatrix}
        \frac{1}{2} \\ -\frac{1}{2} \\ \frac{1}{2} \\ \frac{1}{2}
    \end{bmatrix}.
\end{align}
\end{lem}

% \begin{lem}\label{lem:minmax}
% Let $W ^{\min}, b ^{\min},W ^{\max},$ and $b ^{\max}$ be defined as:
% % The functions $\min(x,y)$ and $\max(x,y)$ can be specified as ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$ such that
% \begin{align}
%     W ^{\min} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             1 & -1 \\
%             -1 & 1 \\
%             -1 & -1
%     \end{bmatrix},
%     b^{\min} = 
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & -\frac{1}{2} & -\frac{1}{2}
%     \end{bmatrix}
% \end{align}
% \begin{align}
%     W^{\max} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             -1 & -1 \\
%             -1 & 1 \\
%             1 & -1
%     \end{bmatrix},
%      b^{\max} =
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & \frac{1}{2} & \frac{1}{2}
%     \end{bmatrix}.
% \end{align}
% The maximum or minimum of a pair of numbers can be computed using a ReLU network with width of $4$ and a depth of $2$ as:
% \begin{align}
% \min(x,y) &= \relu \left(  W ^{\min} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T b^{\min} \\ 
% \max(x,y) &= \relu \left(  W ^{\max} \begin{bmatrix} x \\ y \end{bmatrix} \right)^T b^{\max}.
% \end{align}
% \end{lem}
% \begin{proof}
%     See Lem. D.3 of \cite{arora2016} and Sec. 3.2 of \cite{ferlez2020}.
% \end{proof}


% \begin{lem}\label{lem:minmax}
% The functions $\min(x,y)$ and $\max(x,y)$ can be specified as ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$ such that
% \begin{align}
%     W ^{\min} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             1 & -1 \\
%             -1 & 1 \\
%             -1 & -1
%     \end{bmatrix},
%     b^{\min} = 
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & -\frac{1}{2} & -\frac{1}{2}
%     \end{bmatrix}
% \end{align}
% and 
% \begin{align}
%     W^{\max} &= 
%     \begin{bmatrix}
%             1 & 1 \\
%             -1 & -1 \\
%             -1 & 1 \\
%             1 & -1
%     \end{bmatrix},
%      b^{\max} =
%     \begin{bmatrix}
%         \frac{1}{2} & -\frac{1}{2} & \frac{1}{2} & \frac{1}{2}
%     \end{bmatrix}.
% \end{align}
% \end{lem}
% \begin{proof}
%     See Lem. D.3 of \cite{arora2016} and Sec. 3.2 of \cite{ferlez2020}.
% \end{proof}
By applying Lemma \ref{lem:minmax} recursively, one can implement multi-element min(max) operations with ReLU networks and construct the following bound:
% It is straightforward to generalize Lem. \ref{lem:minmax} to implement multi-element min(max) operations with ReLU networks \cite{arora2016, ferlez2020}.
\begin{cor}
\label{cor:relu_minmax_size}
The minimum (maximum) of $N$ numbers can be represented exactly with a ReLU network with width and depth bounded by $4 \cdot \bigl \lceil \frac{N}{2} \bigr \rceil$ and $2 \cdot \lfloor \log_{2} N \rfloor $, respectively.
\end{cor}
% \begin{proof}
%     See Lem. D.3 of \cite{arora2016} and Sec. 3.2 of \cite{ferlez2020}.
% \end{proof}
One can apply these results to prove the following theorem:
\begin{thm}
\label{thm:relu_sdf_network}
Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes in $\R^2$ for each $j \in \J$ where $\J$ has a finite number of elements in it.
Let $\Obs = \bigcup_{j \in \J} \Oj$.
Let $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
Suppose that for each $j \in \J$, $\Ojz$ has $N_j$ vertices.
Then the signed distance between $\Z$ and $\Obs$ can be represented \textbf{exactly} using a ReLU network
width and depth bounded by  $4 \cdot \bigl \lceil \sum_{j \in \J} \frac{\sum_{j \in \J} N_j }{2} \bigr \rceil + 8$ and $2 \cdot \lfloor \log_{2}  ( \sum_{j \in \J} N_j ) \rfloor + 4$, respectively.
% with $2 \sum_{ j \in \J} N_j$ ReLU operations. 
% The signed distance between a collection of zonotopes can be represented \textbf{exactly} using a ReLU network.
\end{thm}
\begin{proof} 
Let $V_j$ be the set of vertices of $\Ojz$ ordered in counterclockwise fashion and $\{h_{i,j}\}_{i=1}^{N_j}$ be the set of line segments between consecutive vertices in $V_j$.
Using Theorem \ref{thm:exact_rdf}, one can compute the signed distance between $\Z$ and $\Obs$ by applying Lemma \ref{lem:minmax}, if one can compute $\dist(\cz; h_{i,j})$.

Let $v_{i,j}$ and $v_{i+1,j}$ be the vertices corresponding to line segment $h_{i,j}$.   
Let $H_{i,j}(\tau) = v_{i,j} + (v_{i+1,j} - v_{i,j})\tau$, which is the line that extends $h_{i,j}$.

The projection of $\cz$ onto $H_{i,j}$ is
\begin{equation}
    \hat{t}_{i,j} = \frac{(\cz - v_{i,j})^T(v_{i+1,j} - v_{i,j})}{(v_{i+1,j} - v_{i,j})^T (v_{i+1,j} - v_{i,j})}.
\end{equation}
Note that $H_{i,j}(\hat{t}_{i,j})$ is the point on $H_{i,j}$ closest to $\cz$, but it may not be on the line segment $h_i$.
Therefore it is necessary to project $\hat{t}_{i,j}$ onto the interval $[0,1]$:
\begin{equation}\label{eq:segment_projection}
     t_{i,j}^{\ast} = \min (\max (\hat{t}_{i,j}, 0), 1).
\end{equation}
One can compute \eqref{eq:segment_projection} using Lemma \ref{lem:minmax} by performing $2$ ReLU operations, which requires a ReLU network of width and depth bounded by $8$ and $4$, respectively. 
Then the distance between $\cz$ and $h_i$ is 
\begin{equation}\label{eq:segment_distance}
    \dist(\cz; h_i) = \| \cz - (v_i + (v_{i+1} - v_i)t_i^{\ast})\|_{2}.
\end{equation}

The result follows by noting that to compute the signed distance between $\Z$ and $\Obs$ using \eqref{eq:rdf}, one needs to perform \eqref{eq:segment_projection} once for each line segment in $\Ojz$ and noting that $\Obs$ has $\sum_{j\in \J} N_j$ line segments.
\end{proof}

% \begin{thm}
% \label{thm:relu_sdf_network}
% Let $\Z = \zonocg{\cz}{\Gz}$ and $\Oj = \zonocg{\coj}{\Goj}$ be zonotopes in $\R^2$ for each $j \in \J$ where $\J$ has a finite number of elements in it.
% Let $\Obs = \bigcup_{j \in \J} \Oj$.
% Let $\Ojz = \zonocg{\coj}{[\Gz,\Goj]}$.
% Suppose that for each $j \in \J$, $\Ojz$ has $N_j$ vertices.
% Then the signed distance between $\Z$ and $\Obs$ can be represented \textbf{exactly} using a ReLU network with $2 \sum_{ j \in \J} N_j$ ReLU operations. 
% % The signed distance between a collection of zonotopes can be represented \textbf{exactly} using a ReLU network.
% \end{thm}
% \begin{proof} 
% Let $V_j$ be the set of vertices of $\Ojz$ ordered in counterclockwise fashion and $\{h_{i,j}\}_{i=1}^{N_j}$ be the set of line segments between consecutive vertices in $V_j$.
% Let $v_{i,j}$ and $v_{i+1,j}$ be the vertices corresponding to line segment $h_i$.   
% As a result of Theorem \ref{thm:exact_rdf}, one can compute the signed distance between $\Z$ and $\Obs$ by applying Lemma \ref{lem:minmax}, if one can compute $\dist(\cz; h_{i,j})$.

% Let $H_{i,j}(\tau) = v_{i,j} + (v_{i+1,j} - v_{i,j})\tau$, which is the line that extends $h_{i,j}$.
% Then the projection of $\cz$ onto $H_{i,j}$ is
% \begin{equation}
%     \hat{t}_{i,j} = \frac{(\cz - v_{i,j})^T(v_{i+1,j} - v_{i,j})}{(v_{i+1,j} - v_{i,j})^T (v_{i+1,j} - v_{i,j})}.
% \end{equation}
% Note that $H_{i,j}(\hat{t}_{i,j})$ is the point on $H_{i,j}$ closest to $\cz$, but it may not be on the line segment $h_i$.
% Therefore it is necessary to project $\hat{t}_{i,j}$ onto the interval $[0,1]$:
% \begin{equation}\label{eq:segment_projection}
%      t_{i,j}^{\ast} = \min (\max (\hat{t}_{i,j}, 0), 1).
% \end{equation}
% One can compute \eqref{eq:segment_projection} using Lemma \ref{lem:minmax} by performing $2$ ReLU operations. 

% can be computed using Lemma  \ref{lem:minmax}. 
% By Lem. \ref{lem:minmax}, eq \eqref{eq:segment_projection} can be computed with ReLU networks with weights $\Theta^{\min} = (W ^{\min}, b ^{\min})$ and $\Theta^{\max} = (W ^{\max}, b ^{\max})$
% \begin{align}
%     \Tilde{t}_i &= \mathbf{relu}(W^{\max} \cdot \begin{bmatrix}\hat{t}_i \\ 0\end{bmatrix})^T b^{\max}  \\
%     t_i^{\ast} &= \mathbf{relu}(W^{\min} \cdot \begin{bmatrix}\Tilde{t}_i \\ 1\end{bmatrix})^T b^{\min}.
% \end{align}
% Then the distance between $\cz$ and $h_i$ is
% \begin{equation}\label{eq:segment_distance}
%     \dist(\cz; h_i) = \| \cz - (v_i + (v_{i+1} - v_i)t_i^{\ast})\|_{2}.
% \end{equation}
% We then obtain the signed distance between $\Z$ and $\mathcal{O}$ from Thm. \ref{thm:exact_zono} by computing $\underset{i\in \{1,\ldots,N\}}{\min}\: \dist(\cz; h_i)$ with a ReLU network with width and depth bounds given by Cor. \ref{cor:relu_minmax_size}.
% \end{proof}

% \begin{rem}
%     This result can be trivially extended to compute the signed distance to a collection of $M$ zonotopes by batching the computations described in Thm \ref{thm:relu_sdf_network} and passing the output to another ReLU network that computes the minimum of $M$ numbers.
% \end{rem}


\subsection{Trajectory Optimization}


\subsection{Online Operation}


==> sections/old/07_rdf.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%~~~~~~~~~~~~~~~~~~~~~~~Overview of RDFs
\section{Reachability-based Signed Distance Functions}
\label{sec:RDF}
\jon{We can either 1) place this in the prelim section; 2) combine with Neural net section; 3) remove altogether}
% This section defines the signed distance function between sets. 
% Signed distance functions are used in robotics in a variety of applications including representing collision avoidance constraints. 
This section describes how to extend the signed distance function to a distance function between the forward reachable set of a robot and an obstacle. 
This novel distance function, which we call the reachability-based signed distance function (\methodname{}), was introduced in \cite{michaux2023rdf} and  enables us to formulate the collision avoidance problem between a parameterized reachable set and an obstacle as an optimization problem. 

\subsection{Signed Distance Functions}
We begin by defining an unsigned distance function:
\begin{defn}
Given a set $\Omega \subset \mathbb{R}^{\nd}$, the \defemph{distance function} associated with $\Omega$ is defined by
    \begin{equation}
       \dist(x;\Omega) = \min_{y \in \partial\Omega} \|x - y\|.
    \end{equation}
The \defemph{distance between two sets} $\Omega_1, \Omega_2 \subset \mathbb{R}^{\nd}$ is defined by
    \begin{equation}
       \dist(\Omega_1,\Omega_2) = \min_{\substack{x \in \partial\Omega_1 \\ y \in \partial\Omega_2}} \|x - y\|.
    \end{equation}
\end{defn}
\textbf{Notice that this distance function is zero for sets that have non-trivial intersection. 
As a result, this distance function provides limited information for such sets (i.e., it is unclear how much they are intersecting with one another).
To address this limitation, we consider the following definition:}
\begin{defn} Given a subset $\Omega$ of $\mathbb{R}^{\nd}$, the \defemph{signed distance function} $\sdf$ between a point is a map $\sdf: \mathbb{R}^{\nd} \to \mathbb{R}$ defined as
    \begin{equation}
    \sdf(x; \Omega) = 
        \begin{cases}
          \dist(x, \partial\Omega)  & \text{if } x \not \in \Omega \\
          -\dist(x,\partial\Omega) & \text{if } x \in \Omega.
        \end{cases}
\end{equation}
The \defemph{signed distance between two sets} $\Omega_1, \Omega_2 \subset \mathbb{R}^{\nd}$ is defined as
    \begin{equation}
    \sdf(\Omega_1,\Omega_2) = 
        \begin{cases}
          \dist(\Omega_1,\Omega_2)  & \text{if } \Omega_1 \cap \Omega_2 = \emptyset  \\
          -\dist(\Omega_1,\Omega_2) & \text{otherwise}.
        \end{cases}
\end{equation}
\end{defn}
% \begin{itemize}
%     \item Signed distance functions are a common representation in robotics.
%     \item In this section we give a brief overview of signed distance functions and describe some of their notable properties.
%     \item In the context of motion planning the SDF has been used to compute the distance between a single configuration of a robot and a static obstacle \cite{XXX}.
%     \item We then introduce the reachability-based distance function, which represents the distance to a swept volume.
% \end{itemize}


\subsection{Reachability-Based Signed Distance Functions}
This subsection describes the reachability-based distance function as the signed distance function associated with the forward reachable set of the ego vehicle.
% The following sections describe how to overapproximate the forward occupancy and distance calculations with zonotopes using reachability analysis.
\begin{defn}\label{def:rdf_point}
The \defemph{reachability-based distance} function associated with the forward occupancy reachable set $\FO$ is a mapping 
defined by
\begin{equation}
    \rdf(x, \FO) = \min_{j \in \Nj} \rdf_j(x;\FO_j)
\end{equation}
where
$\rdf_j$ is the signed distance function associated with the $j^{th}$ forward occupancy $\FO_j$ such that
\begin{equation}
    \rdf_j(x;\FO_j) = \sdf(x;\FO_j).
\end{equation}
The \defemph{reachability-based distance} between an obstacle $O \subset \mathbb{R}^d$ and the robot's forward occupancy reachable set $\FO$ is defined by
\begin{equation}
    \rdf(O, \FO) = \min_{j \in \Nj} \rdf_j(O, \FO_j).
\end{equation}
\end{defn}
One can use this distance function to formulate trajectory optimization problems as we describe next. \jon{This statement is out of place}



==> sections/symbols.tex <==
\section*{List of Symbols}
\subsection*{Colors}
\begin{itemize}
    \item Red - obstacles
    \item Purple - reachable set
\end{itemize}

\subsection*{Generic Mathematical Symbols}
\begin{itemize}
%   \item $\lambda_j$: indeterminants
\item $\hat{e}_l$
  \item $n$: generic constant
  \item $\mathbb{N}$: natural numbers
  \item $\mathbb{R}^n$: reals 
%   \item $S_i(t)$: sliced reachable set
  \item $X$: a general set and/or metric space
\end{itemize}

\subsection*{Zonotope Symbols}
\begin{itemize}
    \item $Z$: generic zonotope
    \item $Z_1$: generic zonotope
    \item $Z_2$: generic zonotope
    \item $Z_1^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_1$
    \item $Z_2^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_2$
    \item $\beta_i$: zonotope indeterminants
    \item $\beta_{\forall}$: all indeterminants of a zonotope
    \item $c$: zonotope center
    \item $g_i$: ith zonotope generator
    \item $g_{\forall}$: all generators of a zonotope
    \item $\pzgi$: ith PZ coefficient (aka generator)
    \item $G_i$:  ith generator matrix of Matrix zonotope 
    \item $\nhj$: number of halfspaces of $\Pj$
    \item $M$: matrix zonotope
    \item $\pzn$: number of PZ generators
    \item $p_1$: generic point inside poly zonotope
    \item $p_2$: generic point inside poly zonotope
    %   \item $PZ$: generic polynomial zonotope
    \item $\pz{P_1}$: generic polynomial zonotope
    \item $\pz{P_2}$: generic polynomial zonotope
    \item $\Pj$: convexhull of $j$-th link's buffered FRS
    \item $\pz{R_{i-1}^i}$: poly zonotope representation of orientation of frame $i-1$ \textit{wrt} frame i
    \item $\pzv$: indeterminant for polynomial zonotope
    \item $\pzgi$: ith PZ coefficient (aka generator)
    \item $\sigma$: coefficient to be sliced/evaluated
\end{itemize}

\subsection*{SDF Symbols}
\begin{itemize}
  \item $\dist(\cdot)$: distance function
  \item \jon{need a symbol for sdf}
\end{itemize}

\subsection*{Coordinate frames and Transformations}
\begin{itemize}
    \item $p_i$: position of frame $i$ relative to frame $0$
    \item $p_{i-1,i}^i$: position of frame i wrt frame i-1 expressed in frame i \jon{i think this is not needed}
    \item $Q$: configuration space
    \item $R_{i-1}^i$: orientation of frame $i-1$ \textit{wrt} frame $i$
    \item $R_i(q)$: orientation of frame $i$ \textit{wrt} frame $0$
    \item $^Wx$: point $x$ represented in the world frame $W$
    \item $W$: world frame
    \item $W_s$ workspace frame of the robot
  \item $\omega_i^i$: frame i angular velocity wrt frame i
  \item $\dot{\omega}_i^i$: frame i angular acceleration wrt frame i
\end{itemize}

\subsection*{Trajectory Symbols}
\begin{itemize}
    \item $\kscale$: scale for $k$ interval
    \item $i$: time index
    \item $k$: trajectory parameter
    \item $K$: space of trajectory parameters
    \item $\nt$: number of time steps
    \item $j\in\Nq$: $j\in\{1,\cdots,\nq\}$
    \item $i\in\Nt$: $i\in\{1,\cdots,\nt\}$
    \item $h\in\Nhj$: $h\in\{1,\cdots,\nhj\}$
    \item $t$: time
    \item $t_i$: indexed time
    \item $T$: time interval
\end{itemize}

\subsection*{SJO Symbols}
\begin{itemize}
  \item $\pzCjiK$
  \item $\pzuj$
\end{itemize}

\subsection*{SLO Symbols}
\begin{itemize}
  \item 
\end{itemize}

\subsection*{SFO symbols}
\begin{itemize}
    \item 
    \item $c_{j,m}(k)$: The center of the m$^{th}$ sphere on the $j^{th}$ link
    \item $j$: index for specifying joint/link
    \item $\ell_{j,m}(k)$:
    \item $p_{j,1}$: Link $j$'s cap that is closer to the base in the kinematic tree. Also the center of joint $j$. 
    \item $p_{j,2}$: Link $j$'s cap that is closer to the ee in the kinematic tree. Also the center of joint $j+1$.
    \item $p_{j,2} = p_{j+1,1}$ \jon{correct?}
    \item \jon{Maybe we should just use $p_j(k)$ and $p_{j+1}(k)$}
    \item \jon{Should we label all the sphere centers with $c$? Right now the end caps have label $p$}
    \item $r_{j,m}(k)$: The radius of the m$^{th}$ sphere on the $j^{th}$ link
    \item $s(k)$: \jon{I think this symbol depends on the specific joint/link?}
    \item $s'(k)$: \jon{I think this symbol depends on the specific joint/link?}
    \item \adam{thinking about it after crappily writing the section, we should split the SFO to two parts - the Spherical Joint Occupancy, and the Spherical Link Occupancy. As such, we may want separate symbols for the joint center\&radii and the corresponding link ones. maybe a superscript $(l)$ or $(j)$, like $r^{l}_{j,m}$?}
    \item \adam{use $c$, $r$ for joints, $\bar{c}$, $\bar{r}$ for links, subscript tjm}
    
    \item $j$: index for specifying link
    \item $t$: index for specifying time interval
    \item $m \in \{1, 2\}$: index for specifying cap sphere of links, or the joint spheres in the Spherical Joint Occupancy. $1$ is closer to the base in the kinematic tree. $2$ is closer to the end effector in the kinematic tree.
    \item $i$: index for specifying the sphere on the link in the Spherical Link Occupancy
    \item $\mathbf{C}_{t,j,m}$: PZ for the center of joint sphere $m$ in the Joint Spherical Occupancy for link $j$ at the $t^{th}$ time interval.
    \item $c_{t,j,m}$: Some point center of joint sphere $m$ in the Joint Spherical Occupancy for link $j$ at the $t^{th}$ time interval, sliced from $\mathbf{C}_{t,j,m}$.
    \item $r_{t,j,m}$: Radius of the respective joint sphere.
    \item $S_{t,j,m} = (c_{t,j,m}, r_{t,j,m})$: Joint spheres for link $j$ at time interval $t$.
    \item $\mathbf{S}_{t,j,m} = (\mathbf{C}_{t,j,m}, r_{t,j,m})$: Spherical Joint Occupancy for joint $m$ related to link $j$ at time interval $t$.
    \item $S_{t,j,2} = S_{t,j+1,1}$ and $\mathbf{S}_{t,j,2} = \mathbf{S}_{t,j+1,1}$
    \item $\bar{c}_{t,j,\ell}(k)$: Center of the $i^{\text{th}}$ sphere on the $j^{\text{th}}$ link for the $t^{\text{th}}$ time interval in the Spherical Link Occupancy
    \item $\bar{r}_{t,j,\ell}(k)$: Radius of the $i^{\text{th}}$ sphere on the $j^{\text{th}}$ link for the $t^{\text{th}}$ time interval in the Spherical Link Occupancy
    \item $\bar{S}_{t,j,\ell} = (\bar{c}_{t,j,\ell}, \bar{r}_{t,j,\ell})$: Joint spheres for link $j$ at time interval $t$.
    \item \adam{$c$ is used for both the sphere centers and the centers of the joint spheres}
\end{itemize}



\newpage

==> theory/vertex_enumeration.tex <==
\begin{thm}
\label{thm:relu_sdf_network}
Let $\Z = \zonocg{c}{G}$ be a zonotope with $m$ generators $g_1, \cdots, g_m$. 
Assume the generators are sorted in ascending order such that the $y$-value of every generator is nonzero and no two generators have the same direction. 
Then Alg. \ref{alg:vertex_enumeration} produces the vertices of $Z$.
\end{thm}
\begin{proof} 
Let $C$ be the coefficient matrix and $V = \{v_1, \cdots, v_{2m}\}$ be the set of vertices computed by Alg. \ref{alg:vertex}.
We will prove $Z = \conv(V)$.
Let $p \in \conv(V)$ be arbitrary. 
Then there exist non-negative $\sigma_1, \cdots, \sigma_{2m}$, with $\sum_{i=1}^{2m} \sigma_j = 1$, such that $p = \sum_{i=1}^{2m} \sigma_i v_i$.
\jon{I'm taking a little license with Carathéodory's theorem by implicitly assuming that $2m-4$ coefficients are zero}
The point $p$ can be rewritten as
\begin{align}
    p &= \sum_{i=1}^{m} \sigma_i (c + \sum_{j=1}^{m} C(i,j) g_j) + \sum_{i=1}^{m} \sigma_{m+i} (c - \sum_{j=1}^{m} C(i,j) g_j) \nonumber \\
    &= c + \sum_{j=1}^{m}  \underbrace{ \Bigl( \sum_{i=1}^{m} (\sigma_i - \sigma_{m+i}) C(i,j) \Bigr) }_{\beta_j} g_j \nonumber \\
    &= c + \sum_{j=1}^{m} \beta_j g_j.
\end{align}
Since each $\beta_j \in [-1, 1]$, this implies $p \in \Z$ and $\conv(V) \subset \Z$.

Now let $p \in \Z$ be arbitrary. 
Then $p= c + \sum_{j=1}^{m} \beta_j g_j$ such that each $\beta_j \in [-1,1]$.
We must show that there exist non-negative $\sigma_1, \cdots, \sigma_{2m}$, with $\sum_{i=1}^{2m} \sigma_j = 1$, such that
\begin{equation}
    \beta_j = \sum_{i=1}^{m} (\sigma_i - \sigma_{m+i}) C(i,j).
\end{equation}
For $i=1,\cdots, 2m$, we rewrite $\sigma_i = \sigma_i^{+} - \sigma_i^{-}$ with the additional constraint $\sigma_i^{-} = 0$.
This leads to an under-determined system of equations:
\begin{equation}
    \label{eq:indeterminant_conv}
    \begin{bmatrix}
            \mathbf{\beta} \\
            1 \\
            \mathbf{0}_{2m \times 1}
    \end{bmatrix}
    =\begin{bmatrix}
            C & -C & \mathbf{0}_{m \times m} & \mathbf{0}_{m \times m}  \\
            \mathbf{1}_{1\times m} &  \mathbf{1}_{1\times m} & \mathbf{0}_{1\times m} & \mathbf{0}_{1\times m} \\
            \mathbf{0}_{m \times m}&  \mathbf{0}_{m \times m} & I_{m \times m} & \mathbf{0}_{m \times m} \\
            \mathbf{0}_{m \times m} &  \mathbf{0}_{m \times m} & \mathbf{0}_{m \times m} & I_{m \times m} 
    \end{bmatrix}
    \begin{bmatrix}
            \sigma^{+} \\
            \sigma^{-}
    \end{bmatrix}.
\end{equation}
Because the above matrix is rank deficient with linearly independent rows, infinitely many solutions exist.
Therefore $p \in \conv(V)$ and $\Z \subset \conv(V)$.
Thus $\Z = \conv(V)$.
\end{proof}
